An Electronically Non-Adiabatic Generalization of Ring Polymer Molecular Dynamics

In this thesis I generalize Ring Polymer Molecular Dynamics (RPMD) rate theory to electronically non-adiabatic systems, followed by application to two one-dimensional curve crossing models and a multidimensional spin-boson model.

==> sum.tex <==
\section*{Summary}
% Explanatory sentence
In this thesis I generalize Ring Polymer Molecular Dynamics (RPMD) rate theory to electronically non-adiabatic systems, followed by application to two one-dimensional curve crossing models and a multidimensional spin-boson model.

% Explain the extension of RPMD rate theory and importance of non-adiabatic effects
Non-adiabatic effects, where the reactant moves on more than one electronic potential energy surface, are of fundamental importance to numerous branches of chemistry and biology, ranging from quantum dissipation to photosynthesis. RPMD rate theory uses the classical isomorphism to model a quantum mechanical system as many copies of a classical system connected by harmonic springs, forming a ring polymer necklace. By evolving the ring polymer with classical molecular dynamics through an extended classical phase space, the RPMD reaction rate can be calculated. RPMD rate theory is independent of the location of the choice of dividing surface between between products and reactants, and reduces to classical rate theory in the high temperature limit. Here I extend RPMD rate theory to include electronically non-adiabatic effects, leading to a new expression for the potential energy which the ring polymer experiences. 

Numerous desirable features of the non-adiabatic ring polymer potential are illustrated, such as physically plausible results in the high temperature limit for both widely separated and degenerate electronic states. In the limit of a single electronic potential energy surface the conventional adiabatic RPMD potential is recovered, and for system whose Hamiltonian can be separated into electronically coupled and electronically independent components, only the electronically coupled part need be considered using the more computationally demanding non-adiabatic ring polymer potential.

% Application to a 1-D model - procedure and results
The generalisation of RPMD rate theory to non-adiabatic systems is then applied to two one-dimensional Landau-Zener curve crossing models, initially a symmetric model where the optimum dividing surface is evident by symmetry, and then an asymmetric model where the optimum dividing surface is calculated variationally. Thermal RPMD reaction rates and classical rates are calculated over a wide temperature range for both the electronically coupled model, and the adiabatic model where the reactant moves solely on the lower potential energy surface. Exact quantum rates are also available for comparison. The RPMD reaction rates show agreement with exact quantum results to within a factor of two in the symmetric model, even in deep tunneling at 100 K, when the classical rate is in error by many orders of magnitude. For the asymmetric model, RPMD rate theory is an even better approximation to the exact quantum rate, and in both cases the error of the RPMD rate from the quantum rate in the non-adiabatic system is comparable to that of the adiabatic system.

% Application to the spin-boson model - procedure and results
The spin-boson model is then considered, which consists of a spin system bilinearly coupled to a harmonic bath. It has applications ranging from electron transfer in solution to wavepacket dynamics, and a variety of quantum exact and approximate reaction rates are available for comparison. In this thesis the bath is defined by the Debye spectral density, whose long frequency tail leads to the mass of the reaction co-ordinate vanishing in the limit of an infinite number of bath modes. 

The non-adiabatic form of RPMD rate theory is extended to multidimensional systems, followed by a Bennett-Chandler factorisation where the rate calculation is split into a purely statistical Quantum Transisiton State Theory (QTST) calculation and a dynamical (transmission coefficient) calculation. I find that the QTST rate is undefined for the spin-boson model with the Debye Spectral density, and that the transmission coefficient vanishes in the limit of an infinite number of bath modes. However, by an unusual factorisation of the RPMD reaction rate into the probability density of ring polymer centroids at the dividing surface and the flux of positive-momentum centroids which are found in the product region at long time, the RPMD rate is calculable as the product of two convergent factors. Furthermore, the RPMD reaction rate is closer to the exact quantum rate than almost all other approximate methods which are available for comparison. 
